Service Differentiation and Fair Sharing in Distributed Quantum Computing

In the future, quantum computers will become widespread and a network of quantum repeaters will provide them with end-to-end entanglement of remote quantum bits. As a result, a pervasive quantum computation infrastructure will emerge, which will unlock several novel applications, including distributed quantum computing, that is the pooling of resources on multiple computation nodes to address problem instances that are unattainable by any individual quantum computer. In this paper, we first investigate the issue of service differentiation in this new environment. Then, we define the problem of how to select which computation nodes should participate in each pool, so as to achieve a fair share of the quantum network resources available. The analysis is performed via an open source simulator and the results are fully and readily available.

==> tables/002-sensitivity.tex <==
\begin{tabularx}{0.8\columnwidth}{*{5}{c}}
    \hline

    Metric &
    $W$ &
    $D$ &
    $k$ &
    $\phi$ \\

    \hline

    \textit{net rate} &
    $\uparrow$ linear &
    $\downarrow$ asynt &
    $\downarrow$ slight &
    $\approx$  \\

    \textit{fidelity} &
    $\uparrow$ steep &
    $\downarrow$ asynt &
    $\approx$ &
    $\approx$ \\

    \textit{visits} &
    $\uparrow$ linear &
    $\downarrow$ asynt &
    $\uparrow$ linear &
    $\downarrow$ exp \\

    \textit{fairness} &
    $\uparrow$ steep &
    $\downarrow$ asynt &
    $\approx$ &
    $\approx$ then $\downarrow$ exp \\

    \hline
\end{tabularx}

==> tables/functions.tex <==
\begin{tabularx}{\columnwidth}{p{0.46\columnwidth}|p{0.47\columnwidth}}
    \hline

    \texttt{last($\mathcal{L}$)} &
    return the last app in the active list \\
 
    \texttt{next($a$,$\mathcal{L}$)} &
    return the subsequent app to $a$
    in the active list $\mathcal{L}$, wrapping around when the end is reached \\

    \texttt{remove\_app($a$,$\mathcal{L}$)} &
    remove the app $a$ from $\mathcal{L}$ and return the next app in the list,
    wrapping around when the end is reached \\

    \texttt{find\_paths($s$,$d$,$k$,$\mathcal{G}$)} &
    returns the set of (up to) $k$ paths from node $s$ to node $d$
    in $\mathcal{G}$ \\

    \texttt{find\_shortest\_path($\mathcal{P}$}) &
    return the shortest
    path in $\mathcal{P}$ \\

    \texttt{remove\_path($p$,$\mathcal{P}$)} &
    remove the path $p$ from the
    set $\mathcal{P}$ \\

    \texttt{add($a$,$p$,$R$,$\mathcal{F}$)} &
    assign the path $p$ to app $a$ with
    gross rate $R$ in the output $\mathcal{F}$; if the same path $p$ is already
    present in $\mathcal{F}$ for app $a$, then $R$ is simply added to the
    gross rate already reserved \\

    \texttt{remove\_capacity($R$, $p$,$\mathcal{C}_e$)} &
    remove the capacity $R$ from
    the capacities $\mathcal{C}_e$ along the path $p$ \\

    \texttt{update\_graph($\mathcal{G}$,$\mathcal{C}_e$)} &
    update $\mathcal{G}$ by removing the edges with vanishing capacity in $\mathcal{C}_e$ \\

    \hline
\end{tabularx}

==> tables/graphs.tex <==
\begin{tabularx}{\columnwidth}{*{5}{p{0.15\columnwidth}}}
    \hline

    &
    $\mu=100,$ $\tau=15$~km &
    $\mu=100,$ $\tau=20$~km &
    $\mu=50,$ $\tau=15$~km &
    $\mu=50,$ $\tau=20$~km \\

    \hline

    \textit{Capacity} &
    159k &
    257k &
    47k &
    67k \\

    \textit{Num edges} &
    792 &
    1282 &
    232 &
    331 \\

    \textit{Max degree} & 
    16 &
    24 &
    9 &
    13 \\

    \textit{Diameter} &
    8 &
    5 &
    10 &
    6 \\

    \hline
\end{tabularx}

==> tables/metrics.tex <==
\begin{tabularx}{\columnwidth}{lX}
    \hline

    \thead{Metric} &
    \thead{Definition} \\

    \hline

    \textit{net rate} &
    sum of the net rates assigned to peers, in Bell pairs/s \\

    \textit{fidelity} &
    \req{fidelity:perfect} weighted on the net rates assigned to peers \\

    \textit{visits} &
    loop counter of Step~1-Step~6 in \rsec{cont:apps} \\

    \textit{fairness} &
    Raj Jain's index on net rates $\left(\bar{r}\right)^2/\left(\bar{r^2}\right)$ \\

    \hline
\end{tabularx}

==> tables/traffic.tex <==
\begin{tabularx}{\columnwidth}{*{3}{p{0.3\columnwidth}}}
    \hline

    \thead{} &
    \thead{Flows} &
    \thead{Apps} \\

    \hline

    \textit{Nodes involved} &
    source + destination &
    host + set of peers \\

    \textit{Rate requirement} &
    constant Bell rate &
    elastic Bell rate \\

    \textit{Fidelity requirement} &
    strict &
    flexible \\

    \textit{Session duration} &
    user-driven &
    depends on allocation \\

    \textit{QoS} &
    guaranteed upon admission &
    best-effort \\

    % \textit{Priority} &
    % user-driven &
    % user- and system-driven \\

    \hline
\end{tabularx}
